Diverse and Effective Synthetic Data Generation for Adaptable Zero-Shot Dialogue State Tracking

We demonstrate substantial performance gains in zero-shot dialogue state tracking (DST) by enhancing training data diversity through synthetic data generation. Existing DST datasets are severely limited in the number of application domains and slot types they cover due to the high costs of data collection, restricting their adaptability to new domains. This work addresses this challenge with a novel, fully automatic data generation approach that creates synthetic zero-shot DST datasets. Distinguished from previous methods, our approach can generate dialogues across a massive range of application domains, complete with silver-standard dialogue state annotations and slot descriptions. This technique is used to create the D0T dataset for training zero-shot DST models, encompassing an unprecedented 1,000+ domains. Experiments on the MultiWOZ benchmark show that training models on diverse synthetic data improves Joint Goal Accuracy by 6.7%, achieving results competitive with models 13.5 times larger than ours.

==> latex/xw_analysis.tex <==





\begin{table*}[htbp]
    \centering
    \resizebox{0.9\textwidth}{!}{%
    \begin{tabular}{p{5em}|p{10em}|p{30em}|p{1em}}
    \toprule
        \bf Error & \bf Definition & \bf Example & \bf \# \\
        \midrule
        Agent Value Miss & No value is outputted for the indicated slot, even though the information is present in the system's turns. & 
        \begin{tabular}[t]{p{29em}}
        % A: i am planning my trip to cambridge and looking for a place to dine that is in the centre and is in the expensive price range \\
        B: bedouin servers african food and is in the centre of town in the expensive price range . would you like their phone number , or should i book a reservation ? \\
        A: please book a reservation for wednesday at 20:00 for 5 . \\
        % i was unable to book that time slot for you . is there a different day or time that you would be interested in going ?"
        \\
        \texttt{restaurant name: None} \\
        \end{tabular} & 13 \\
        
        \midrule
        No preference & Indications of no preference are inappropriately understood, either by failing to recognize when no preference is given or by incorrectly interpreting an indication of no preference from the dialogue. & 
        \begin{tabular}[t]{p{29em}}
        A: are there any 1 star hotel -s with free parking ? \\
        B: i am sorry , i cannot find any hotel -s that meet your criteria . would you like to search again ? \\
        A: i am looking for a guest house with free parking , preferably 1 star . \\
        B: sorry , i am not finding anything . want to change to a hotel ? \\
        A: what about guest houses ? \\
        \\
        \texttt{hotel parking: any} \\
        \end{tabular} & 13 \\
        
        \midrule
        Value Change & The appropriate value for the indicated slot has been updated in the dialogue turn, but the predicted value remains as the original.  & 
        \begin{tabular}[t]{p{29em}}
        A: i am looking for a place to dine in the centre that serves jamaican food. \\
        B: i am sorry , i am not finding any place that serves jamaican food in the centre of town . would you like to try another area ? \\
        A: that is fine , how about a place that serves indian food ? \\
        \\
        \texttt{restaurant food: jamaican} \\
        \end{tabular} & 10 \\
        
        \midrule
        Hallucination & A value is predicted for the indicated slot that does not exist in the dialogue. & \begin{tabular}[t]{p{29em}}
        % A: i am looking for a train from cambridge to birmingham new street .
        % B: the next train leaving from cambridge for birmingham new street departs friday at 5:01 , and will arrive by 7:44 .
        A: i need a train that departs after 08:30 on friday . \\
        B: i have a train leaving cambridge arriving at birmingham new street on friday at 9:01 . would you like me to book this for you ? \\
        A: yes please , that sounds perfect . \\
        % B: and how many tickets will you need for your trip ? \\
        % A: actually , i do not need booking . please just give me the train s travel time and price . \\
        % B: the travel time is 163 minutes , and the price is 75.10 pounds . how else can i help ? \\
        % A: no thank you . not at this time . \\
        \\
        \texttt{train leave at: after 16:30}
        \end{tabular} & 9 \\
        
        \midrule
        Miss & No value is outputted for the indicated slot, even though the information is present in the user's turns. & 
        \begin{tabular}[t]{p{29em}}
        A: are there any guest houses in the east ? \\
        B: there are 6 guest houses in the east . do you have a preference on price? \\
        A: it needs to be cheap . \\
        \\
        \texttt{hotel area: None}
        \end{tabular} & 7 \\
        
        \midrule
        Wrong Value & Information in the dialogue is incorrectly attributed to the indicated slot. & 
        \begin{tabular}[t]{p{29em}}
        A: hey , are there any interesting attractions in towncentre today ?
        \\
        \texttt{attraction type: interesting}
        \end{tabular} & 6 \\
        
        \midrule
        Other & Errors not explained by any of the other error patterns. &
        \begin{tabular}[t]{p{29em}}
        A: i am looking for a 3 star hotel in cambridge with free wifi \\
        B: there are 5 hotel -s that meet that criteria . do you have a location or price range in mind ? \\
        A: i would like something cheap . \\
        B: unfortunately , none of the cheap hotel -s have free wifi . would you prefer to try a different price range or go with a hotel without free wifi ? \\
        A: how about a hotel with a 4 star rating ? \\
        \\
        \texttt{hotel internet: no} \\
        \end{tabular} 
        & 16 \\

        \midrule
        Correct & The predicted value for the indicated slot is correct, but is missing from the gold annotations in MultiWOZ due to an annotation mistake. & 
        \begin{tabular}[t]{p{29em}}
        A: i am looking for information on a hotel called warkworth house . \\
        B: i got it . may i get the day youd like to move in so i can book
        \\
        \texttt{hotel type: hotel} \\
        \end{tabular} & 26 \\
 
    \bottomrule
    \end{tabular}%
    }
    \caption{Error analysis of DSG5K Zero-shot pretrained model Llama-PT on MultiWOZ}
    \label{tab:dsg5k-pretrained-0shot-error-analysis}
\end{table*}
